Human-Variability-Respecting Optimal Control for Physical Human-Machine Interaction

Physical Human-Machine Interaction plays a pivotal role in facilitating collaboration across various domains. When designing appropriate model-based controllers to assist a human in the interaction, the accuracy of the human model is crucial for the resulting overall behavior of the coupled system. When looking at state-of-the-art control approaches, most methods rely on a deterministic model or no model at all of the human behavior. This poses a gap to the current neuroscientific standard regarding human movement modeling, which uses stochastic optimal control models that include signal-dependent noise processes and therefore describe the human behavior much more accurate than the deterministic counterparts. To close this gap by including these stochastic human models in the control design, we introduce a novel design methodology resulting in a Human-Variability-Respecting Optimal Control that explicitly incorporates the human noise processes and their influence on the mean and variability behavior of a physically coupled human-machine system. Our approach results in an improved overall system performance, i.e. higher accuracy and lower variability in target point reaching, while allowing to shape the joint variability, for example to preserve human natural variability patterns.

==> 1_tex/img/HRVC_system.tex <==

 \definecolor{shadecolor}{rgb}{0.92,0.92,0.92}

\tikzstyle{block} = [rectangle, draw, text width=2cm, text centered, minimum height=1.5cm]
 \tikzstyle{box} = [rectangle, draw, fill=shadecolor, text width=9em, text centered, rounded corners, minimum height=4em]
\tikzstyle{noise} = [rectangle, draw, text width=1.5cm, text centered, minimum height=0.8cm]
\tikzstyle{noiseS} = [rectangle, draw, text width=1cm, text centered, minimum height=0.8cm]
\tikzstyle{plus} = [circle, draw, text width=0.1cm, text centered]
 \tikzstyle{frame} = [rectangle, dashed, draw, text width=9em, text centered, minimum height=4em]


\tikzstyle{line} = [draw, -latex']

\usetikzlibrary{arrows}
\begin{tikzpicture}
 
 %system
\node[block, fill=shadecolor, text width=5cm, text centered, minimum height=2cm] (system) at (3.5,1.75) {Biomechanics \\ $\boldsymbol{x}_{t+1}= \boldsymbol{A} \boldsymbol{x}_t + \boldsymbol{z}_{\mathrm{H},t} + \boldsymbol{z}_{\mathrm{A},t}$ };
%$ \boldsymbol{x}_{t+1} = \boldsymbol{f} ( \boldsymbol{x}_t, \boldsymbol{u}_t, t)$
%{Biomechanics \\ $\boldsymbol{x}_{t+1}= \boldsymbol{A} \boldsymbol{x}_t + \boldsymbol{B}_{\mathrm{A}} \boldsymbol{u}_{\mathrm{A},t} $ \\ $ +\boldsymbol{B}_{\mathrm{H}} \boldsymbol{u}_{\mathrm{H},t}  + \boldsymbol{\xi}_t + \sum_i \varepsilon_t^i \boldsymbol{C}_i \boldsymbol{u}_{\mathrm{H},t} $ };


%Box Human
 %inner xsep = 5.5cm, inner ysep=4cm, xshift=-0.5cm
\node[box,  inner xsep = 5.5cm, inner ysep=2.75cm] (boxH) at (-7.5,4.5) {};
 \node [draw=none, anchor=north west, align = right] at (boxH.north west) {Human};
  
  
%Blocks Human
\node[block,  text width=4.5cm] (estimateH) at (-9.5,5.5) {Estimation \\ $\hat{\boldsymbol{x}}_{\mathrm{H},t+1}=\boldsymbol{A} \hat{\boldsymbol{x}}_{\mathrm{H},t}+ \boldsymbol{B}_\mathrm{H} \boldsymbol{u}_{\mathrm{H},t}$ \\ $+\boldsymbol{K}_{\mathrm{H},t}\left(\boldsymbol{y}_{\mathrm{H},t}- \boldsymbol{H}_{\mathrm{H}} \hat{\boldsymbol{x}}_{\mathrm{H},t}\right)$};
%\node[block] (perceptH) at (-7,5.5) {Perception};
\node[block, text width=3cm] (controlH) at (-12.5,3.5) {Control law \\ $\boldsymbol{u}_{\mathrm{H},t} = - \boldsymbol{L}_{\mathrm{H},t} \hat{\boldsymbol{x}}_{\mathrm{H},t} $};

\node[plus] (plusPercept) at (-5,5.5) {};
%Arrows Human
\path[line] (plusPercept) -- (estimateH)node[midway, xshift=0.25cm, yshift=0.25cm](yH){$\boldsymbol{y}_{\mathrm{H},t}$};
\path[line] (estimateH) -- (controlH.north |- estimateH)node[midway, yshift=0.25cm, xshift=-0.25cm](hatxH){$\hat{\boldsymbol{x}}_{\mathrm{H},t}$} -- (controlH);  
\path[line] (controlH) -- (estimateH.south |- controlH)node[midway, yshift=0.25cm, xshift=0cm](uH){$\boldsymbol{u}_{\mathrm{H},t}$} -- (estimateH);  

%Feedback Human
\node (aidSys) at (6.5,1.75) {};
\node[noise] (H_H) at (-3,5.5) {$\boldsymbol{H}_\mathrm{H}$};

\path[line] (system) -- (aidSys.center) -- (H_H.east -| aidSys.center) -- (H_H);%
\path[line] (H_H) -- (plusPercept);
%\path[line] (plusPercept) -- estimateH);

%Perception noise 
\node[noise] (mulPercept) at (-3,6.5) {$\sum_i \epsilon_t^i \boldsymbol{D}_i $};
\node[noiseS] (addPercept) at (-5,6.5) {$\boldsymbol{\omega}_t$};

%Perception arrow in
\node (aidNPIn) at (-0.75,5.5) {};
\path[line] (aidNPIn.center) -- (mulPercept.east -| aidNPIn.center) -- (mulPercept);

%Perception arrow out
\path[line] (mulPercept.west) -- (plusPercept)node[yshift=0cm](plus1){$+$};
\path[line] (addPercept.south) -- (plusPercept);

%Control noise
%helper-nodes
\node[plus] (plusControl) at (-2.5,3.5) {};

%noise
\node[noise] (B_H) at (-5,3.5) {$\boldsymbol{B}_\mathrm{H}$};
\node[noise] (mulControl) at (-5,2.5) {$\sum_i \varepsilon_t^i \boldsymbol{C}_i $};
\node[noiseS] (addControl) at (-2.5,2.5) {$\boldsymbol{\xi}_t$};
%arrow
\path[line] (controlH) -- (B_H);
\path[line] (B_H) -- (plusControl)node[yshift=0cm](plus2){$+$};
\path[line] (mulControl.east) -- (plusControl);
\path[line] (addControl.north) -- (plusControl);

\node (aidNCIn) at (-6.25,3.5) {};
\path[line] (aidNCIn.center) -- (mulControl.west -| aidNCIn.center) -- (mulControl);


%human-->system
\node (aidH) at (0.5,3.5) {};
\node (sysInH) at (1,2.0) {};

\path[line] (plusControl)-- (aidH.center)node[midway, xshift=1.25cm, yshift=0.25cm](zH){$\boldsymbol{z}_{\mathrm{H},t}$} -- (sysInH.west -| aidH.center) -- (sysInH);


%-----------------------


%Box Aut
 %inner xsep = 5.5cm, inner ysep=4cm, xshift=-0.5cm
\node[box,  inner xsep = 5.5cm, inner ysep=2.25cm] (boxA) at (-7.5,-0.75) {};
 \node [draw=none, anchor=north west, align = right] at (boxA.north west) {Automation};
  
%Blocks Aut
\node[block,  text width=4.5cm] (estimateA) at (-8.5,-2) {Estimation \\ $\hat{\boldsymbol{x}}_{\mathrm{A},t+1}=\boldsymbol{A} \hat{\boldsymbol{x}}_{\mathrm{A},t}+ \boldsymbol{B}_\mathrm{A} \boldsymbol{u}_{\mathrm{A},t} $\\$+\boldsymbol{K}_{\mathrm{A},t}\left(\boldsymbol{y}_{\mathrm{A},t}- \boldsymbol{H}_{\mathrm{A}} \hat{\boldsymbol{x}}_{\mathrm{A},t}\right)$};
\node[block] (perceptA) at (-2.5,-2) {Perception $\boldsymbol{H}_\mathrm{A}$};

\node[block, text width=3.5cm] (controlA) at (-12,0) {Control law \\ $\boldsymbol{u}_{\mathrm{A},t} = - \boldsymbol{L}_{\mathrm{A},t} \hat{\boldsymbol{x}}_{\mathrm{A},t} $};

\node[noise] (B_A) at (-2.5,0) {$\boldsymbol{B}_\mathrm{A}$};

\path[line] (perceptA) -- (estimateA)node[midway, yshift=0.25cm](yA){$\boldsymbol{y}_{\mathrm{A},t}$};
\path[line] (estimateA) -- (controlA.north |- estimateA)node[midway, yshift=0.25cm](hatxA){$\hat{\boldsymbol{x}}_{\mathrm{A},t}$} -- (controlA);  
\path[line] (controlA) -- (estimateA.south |- controlA)node[midway, yshift=0.25cm](uA){$\boldsymbol{u}_{\mathrm{A},t}$} -- (estimateA);  


%feedback

\path[line] (system) -- (aidSys.center)node[midway, xshift=0.5cm](yA){$\boldsymbol{x}_t$} -- (perceptA.east -| aidSys.center) -- (perceptA);

%human-->system
\node (aidA) at (0.5,0) {};

\node (sysInA) at (1,1.5) {};

\node (sysInH) at (1,1.0) {};

\path[line] (controlA) -- (B_A);
\path[line] (B_A)-- (aidA.center)node[midway, xshift=1cm, yshift=-0.25cm](zH){$\boldsymbol{z}_{\mathrm{A},t}$} -- (sysInA.west -| aidA.center) -- (sysInA);



%FRAMES

\node[frame,  inner xsep = 1.25cm, inner ysep=1.25cm] (framePercept) at (-3.5,5.8) {};
 \node [draw=none, anchor=south west, align = right] at (framePercept.south west) {Perception};

\node[frame,  inner xsep = 1.25cm, inner ysep=1.25cm] (frameAction) at (-3.5,3.2) {};
 \node [draw=none, anchor=north east, align = right] at (frameAction.north east) {Action};



\end{tikzpicture}

==> 1_tex/img/HVROC_procedure.tex <==
% \definecolor{r1}{RGB}{0,150,130}
\definecolor{gray1}{RGB}{242,242,242}
\definecolor{gray2}{RGB}{180,180,180}


\usetikzlibrary{arrows}

\tikzstyle{block} = [rectangle, draw, fill=white,
   text width=2cm, text centered, minimum height=4em]
\tikzstyle{box} = [rectangle, draw, text width=24em, text centered,  minimum height=8em] %fill=gray1, rounded corners,
\tikzstyle{line} = [draw, ->] % [draw, -latex']


\begin{tikzpicture}[node distance = 2cm, auto]
    
  	\node [text width = 4.5cm, align=center ] (ident) at (0,10) { $ \boldsymbol{A}, \boldsymbol{B}_\mathrm{H},  \boldsymbol{B}_\mathrm{A},  \boldsymbol{H}_\mathrm{H},  \boldsymbol{H}_\mathrm{A},$ \\ %$\bigA, \bigB_\mathrm{H}, \bigB_\mathrm{A}, \bigH_\mathrm{H}, \bigH_\mathrm{A},$ \\
  	$\boldsymbol{Q}_{\mathrm{H},t}, \boldsymbol{R}_{\mathrm{H}}, 
  	 \boldsymbol{C}_i, \boldsymbol{D}, \boldsymbol{\Sigma}^{\boldsymbol{\omega}}, \boldsymbol{\Sigma}^{\boldsymbol{\xi}},   $}; 
   	\node [block, text width = 6.5cm] (meanHuman) at (0,8) {$\mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \mathrm{cov}(\boldsymbol{p}_\mathrm{human}) $ using~\eqref{eq:E_human},~\eqref{eq:cov_human}};
   	
   	\node [box, inner xsep = 1cm, inner ysep=3cm, anchor=north] (box) at (0,6.5) {};

	%bilevel block
   	\node [block, text width = 9cm] (calcTop) at (0,5) { \begin{align} 
   	\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	& \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}), \mathrm{cov}(\boldsymbol{p}_\mathrm{human}), \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	\end{align}};

	\node [block, text width = 9cm] (calcBot) at (0,1.5) { $
   	\mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, 
   	\mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC})  $ by Lemma~\ref{lemma}};

	%arrows bi-level
	\node[xshift=-1cm] (anchorTL) at (calcTop.south) {} ;	
	\node[xshift=-1cm] (anchorBL) at (calcBot.north) {};	
	\path[line] (anchorTL.center) -- (anchorBL.center)node[midway, left](q-r) {$\boldsymbol{q}_{\mathrm{A}}, \boldsymbol{r}_{\mathrm{A}} $};

	\node[xshift=1cm] (anchorTR) at (calcTop.south) {};	
	\node[xshift=1cm] (anchorBR) at (calcBot.north) {};	
	\path[line] (anchorBR.center) -- (anchorTR.center)node[midway, right](q-r) {$ \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}) $};
	
	
	%left blocks
	\node [text width = 3cm, align=left] (input) at (-7.5,5) {$\boldsymbol{p}_\mathrm{ref}, \boldsymbol{q}_0, \boldsymbol{r}_0,$ \\
	$\boldsymbol{s} = \begin{bmatrix} s_\mathrm{highMidVar} \\ s_\mathrm{lowMidVar} \\  s_\mathrm{endVar} \\ s_\mathrm{ref} \end{bmatrix}$ };
	
	\path[line] (input) -- (box.west |- input) {};
	
	\node[block] (output) at (0,-1.5) {$\boldsymbol{L}^*_\mathrm{A}$, see~\ref{sec:automation} };
	
	\path[line] (ident) -- (meanHuman);
	\path[line] (meanHuman) -- (box);
	\path[line] (box) -- (output)node[midway](out){$\boldsymbol{q}_{\mathrm{A}}^*, \boldsymbol{r}_{\mathrm{A}}^* $};
	

\end{tikzpicture}


==> 1_tex/img/HVROC_procedure_cov.tex <==
% \definecolor{r1}{RGB}{0,150,130}
\definecolor{gray1}{RGB}{242,242,242}
\definecolor{gray2}{RGB}{180,180,180}


\usetikzlibrary{arrows}

\tikzstyle{block} = [rectangle, draw, fill=white,
   text width=2cm, text centered, minimum height=4em]
\tikzstyle{box} = [rectangle, draw, text width=24em, text centered,  minimum height=8em] %fill=gray1, rounded corners,
\tikzstyle{line} = [draw, ->] % [draw, -latex']


\begin{tikzpicture}[node distance = 2cm, auto]
    
  	\node [text width = 4.5cm, align=center ] (ident) at (0,10) { $ \boldsymbol{A}, \boldsymbol{B}_\mathrm{H},  \boldsymbol{B}_\mathrm{A},  \boldsymbol{H}_\mathrm{H},  \boldsymbol{H}_\mathrm{A},$ \\ %$\bigA, \bigB_\mathrm{H}, \bigB_\mathrm{A}, \bigH_\mathrm{H}, \bigH_\mathrm{A},$ \\
  	$\boldsymbol{Q}_{\mathrm{H},t}, \boldsymbol{R}_{\mathrm{H}}, 
  	 \boldsymbol{C}_i, \boldsymbol{D}, \boldsymbol{\Sigma}^{\boldsymbol{\omega}}, \boldsymbol{\Sigma}^{\boldsymbol{\xi}},   $}; 
   	\node [block, text width = 6.5cm] (meanHuman) at (0,8) {$\mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \mathrm{cov}(\boldsymbol{p}_\mathrm{human}) $ using~\eqref{eq:E_human},~\eqref{eq:cov_human}};
   	
   	\node [box, inner xsep = 1cm, inner ysep=3cm, anchor=north] (box) at (0,6.5) {};

	%bilevel block
   	\node [block, text width = 9cm] (calcTop) at (0,5) { \begin{align}    	
   	\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	& \bigOmega_{\mathrm{HVROC}}^{\bigp}, \bigOmega_{\mathrm{human}}^{\bigp}, \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	%\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	%& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	%& \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}), \mathrm{cov}(\boldsymbol{p}_\mathrm{human}), \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	\end{align}};

	\node [block, text width = 9cm] (calcBot) at (0,1.5) { $
   	\mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, 
   	\bigOmega_{\mathrm{human}}^{\bigp}  $ by Lemma~\ref{lemma}};
   	%\mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC})  $ by Lemma~\ref{lemma}};

	%arrows bi-level
	\node[xshift=-1cm] (anchorTL) at (calcTop.south) {} ;	
	\node[xshift=-1cm] (anchorBL) at (calcBot.north) {};	
	\path[line] (anchorTL.center) -- (anchorBL.center)node[midway, left](q-r) {$\boldsymbol{q}_{\mathrm{A}}, \boldsymbol{r}_{\mathrm{A}} $};

	\node[xshift=1cm] (anchorTR) at (calcTop.south) {};	
	\node[xshift=1cm] (anchorBR) at (calcBot.north) {};	
	\path[line] (anchorBR.center) -- (anchorTR.center)node[midway, right](q-r) {$ \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, \bigOmega_{\mathrm{HVROC}}^{\bigp} $}; %     \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}) $};
	
	
	%left blocks
	\node [text width = 3cm, align=left] (input) at (-7.5,5) {$\boldsymbol{p}_\mathrm{ref}, \boldsymbol{q}_0, \boldsymbol{r}_0,$ \\
	$\boldsymbol{s} = \begin{bmatrix} s_\mathrm{highMidVar} \\ s_\mathrm{lowMidVar} \\  s_\mathrm{endVar} \\ s_\mathrm{ref} \end{bmatrix}$ };
	
	\path[line] (input) -- (box.west |- input) {};
	
	\node[block] (output) at (0,-1.5) {$\boldsymbol{L}^*_\mathrm{A}$, see~\ref{sec:automation} };
	
	\path[line] (ident) -- (meanHuman);
	\path[line] (meanHuman) -- (box);
	\path[line] (box) -- (output)node[midway](out){$\boldsymbol{q}_{\mathrm{A}}^*, \boldsymbol{r}_{\mathrm{A}}^* $};
	

\end{tikzpicture}


==> 1_tex/plots/result_hand0.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=2.344in,
height=2.344in,
at={(1.016in,0.406in)},
scale only axis,
xmin=0,
xmax=42,
xlabel style={font=\color{white!15!black}},
xlabel={Time Steps $t$},
ymin=0,
ymax=0.11,
ytick={  0, 0.1},
ylabel style={font=\color{white!15!black}},
ylabel={E\{$ p_x$\} [$\si{m^2}$]},
axis background/.style={fill=white},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, line width=1.5pt]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0\\
5	5.59211212138388e-05\\
6	0.000246495726334693\\
7	0.000653236759819613\\
8	0.00134904344707812\\
9	0.00239238534491977\\
10	0.00382499929177087\\
11	0.00567172205704975\\
12	0.00794155321378419\\
13	0.0106293632403218\\
14	0.0137178779703596\\
15	0.017179714989012\\
16	0.0209793423757342\\
17	0.0250748868223482\\
18	0.0294197439155017\\
19	0.0339639642073042\\
20	0.0386554169555779\\
21	0.0434407492389395\\
22	0.0482661690064786\\
23	0.0530780948080908\\
24	0.057823730668681\\
25	0.0624516397550478\\
26	0.0669124010023579\\
27	0.0711594302083726\\
28	0.0751500210473039\\
29	0.0788466058842289\\
30	0.0822181570237544\\
31	0.085241565942425\\
32	0.0879027738509271\\
33	0.0901974335489929\\
34	0.0921310091522648\\
35	0.0937183331598806\\
36	0.0949827335805147\\
37	0.0959550972065412\\
38	0.096673030581396\\
39	0.0971797593611696\\
40	0.0975226181278802\\
41	0.0977484537807249\\
42	0.0978972576360758\\
};
\addlegendentry{Human}

\addplot [color=blue, line width=1.5pt]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0.000173768304220472\\
5	0.000683340317127598\\
6	0.00166756185218549\\
7	0.00323699535906196\\
8	0.00541664848686698\\
9	0.00823153178171179\\
10	0.011625417917633\\
11	0.0155128315460071\\
12	0.0197968155841297\\
13	0.0243796782107093\\
14	0.0291693286669784\\
15	0.0340825667166743\\
16	0.0390463649784466\\
17	0.0439978961131831\\
18	0.048883826966211\\
19	0.0536592472128032\\
20	0.0582864751072915\\
21	0.0627338944215354\\
22	0.066974941131081\\
23	0.0709872891308957\\
24	0.0747522241116914\\
25	0.0782542112111682\\
26	0.0814806885448375\\
27	0.0844221199291596\\
28	0.0870723033586118\\
29	0.0894288498076343\\
30	0.0914936725545547\\
31	0.0932733247993308\\
32	0.094779072439055\\
33	0.0960266524845834\\
34	0.0970357445661105\\
35	0.0978292262634884\\
36	0.0984323200884513\\
37	0.0988718110226534\\
38	0.0991753713179742\\
39	0.0993708984709871\\
40	0.0994858928929011\\
41	0.0995456287919089\\
42	0.0995706887604917\\
};
\addlegendentry{HVROC - high var}

\addplot [color=blue, dashed, line width=1.5pt]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	9.89307920793721e-05\\
5	0.00041903952393496\\
6	0.00108132460443249\\
7	0.00219191006666538\\
8	0.00380228053091077\\
9	0.00595466729799208\\
10	0.00863479270417562\\
11	0.0118018021956808\\
12	0.0153994234544624\\
13	0.019363450622284\\
14	0.0236268038914196\\
15	0.0281228075420431\\
16	0.0327872067946526\\
17	0.0375593154750004\\
18	0.0423825736643828\\
19	0.0472047235785056\\
20	0.0519777541500592\\
21	0.0566577226649825\\
22	0.0612045572575331\\
23	0.0655819000809014\\
24	0.0697569993996751\\
25	0.0737006740280303\\
26	0.0773873996577365\\
27	0.0807955670122189\\
28	0.0839079291623268\\
29	0.086712187512065\\
30	0.0892015972198209\\
31	0.0913754469818088\\
32	0.0932392798858805\\
33	0.0948047664287121\\
34	0.0960892306675019\\
35	0.097114891821243\\
36	0.0979079345131613\\
37	0.098497635786773\\
38	0.0989156085874668\\
39	0.0991949915793578\\
40	0.099369565807748\\
41	0.0994711416206144\\
42	0.0995260331214027\\
};
\addlegendentry{HVROC - low var}

\addplot [color=black, line width=1.5pt]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0.000160776601208743\\
5	0.000607548437614762\\
6	0.00143890432847065\\
7	0.00273022715532772\\
8	0.00448914923058673\\
9	0.00673597759578837\\
10	0.0094267611583738\\
11	0.0124986600541397\\
12	0.0158836207056859\\
13	0.0195159072736041\\
14	0.0233360074281092\\
15	0.0272921569173035\\
16	0.0313403837114881\\
17	0.0354437059499642\\
18	0.0395709115789852\\
19	0.0436951990002937\\
20	0.0477928606634806\\
21	0.0518421126889901\\
22	0.0558220690555467\\
23	0.0597118304152342\\
24	0.0634897477396826\\
25	0.0671329602916472\\
26	0.0706172961603029\\
27	0.073917615609213\\
28	0.0770086453422313\\
29	0.0798662631590253\\
30	0.0824690835064294\\
31	0.0848001273852305\\
32	0.0868483336689981\\
33	0.0886096841230968\\
34	0.0900878090508508\\
35	0.0912940350203642\\
36	0.0922469377933815\\
37	0.0929716621635991\\
38	0.0934990904331184\\
39	0.093864656617981\\
40	0.0941068458109622\\
41	0.094263473546483\\
42	0.0943669067277766\\
};
\addlegendentry{LQR}

\end{axis}

\begin{axis}[%
width=2.344in,
height=2.344in,
at={(4.453in,0.406in)},
scale only axis,
xmin=0,
xmax=42,
xlabel style={font=\color{white!15!black}},
xlabel={Time Steps $t$},
ymin=0,
ymax=3.5e-05,
ytick={    0, 1e-05, 2e-05, 3e-05},
ylabel style={font=\color{white!15!black}},
ylabel={cov($ p_x$) [$\si{m^2}$]},
axis background/.style={fill=white}
]
\addplot [color=red, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0\\
5	1.56358589890643e-09\\
6	2.04428152051469e-08\\
7	1.09234727747626e-07\\
8	3.68942915782852e-07\\
9	9.36306166601743e-07\\
10	1.95185625432392e-06\\
11	3.52207892543726e-06\\
12	5.68830659235383e-06\\
13	8.41003756838957e-06\\
14	1.15649014176129e-05\\
15	1.49632679540518e-05\\
16	1.83730234310116e-05\\
17	2.15491270516847e-05\\
18	2.42628550108893e-05\\
19	2.63267648187383e-05\\
20	2.76128122516359e-05\\
21	2.80623588874864e-05\\
22	2.76879489443399e-05\\
23	2.65676396578566e-05\\
24	2.48333120977352e-05\\
25	2.26547854438992e-05\\
26	2.02217316743245e-05\\
27	1.77253678634669e-05\\
28	1.53417154430526e-05\\
29	1.32178772322692e-05\\
30	1.14623180697544e-05\\
31	1.01396063057888e-05\\
32	9.26958626215119e-06\\
33	8.83058352176849e-06\\
34	8.76605712579578e-06\\
35	8.99407948750512e-06\\
36	9.418847620551e-06\\
37	9.94341603647838e-06\\
38	1.04830632893767e-05\\
39	1.09775781730156e-05\\
40	1.13996338787725e-05\\
41	1.17528372410907e-05\\
42	1.20589388304043e-05\\
};
\addplot [color=blue, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0\\
5	1.56358589890643e-09\\
6	2.04428152051469e-08\\
7	1.09234727747626e-07\\
8	3.68289731604705e-07\\
9	9.28398652376796e-07\\
10	1.91461533334136e-06\\
11	3.41595194156767e-06\\
12	5.46880088220104e-06\\
13	8.04822177910865e-06\\
14	1.10664229286358e-05\\
15	1.43803748107208e-05\\
16	1.78074198767198e-05\\
17	2.1145571227808e-05\\
18	2.41948519230265e-05\\
19	2.67767337910249e-05\\
20	2.87497027084175e-05\\
21	3.00198350553468e-05\\
22	3.05461042436956e-05\\
23	3.03407744439301e-05\\
24	2.94654402271971e-05\\
25	2.80232893255273e-05\\
26	2.61482715824448e-05\\
27	2.39920627303377e-05\\
28	2.17099366869822e-05\\
29	1.94468543985676e-05\\
30	1.732522418427e-05\\
31	1.54358162445505e-05\\
32	1.38330696278167e-05\\
33	1.25353804974515e-05\\
34	1.15299906496074e-05\\
35	1.07812598513715e-05\\
36	1.02406137274204e-05\\
37	9.85617281664416e-06\\
38	9.5805179130134e-06\\
39	9.3760272722512e-06\\
40	9.21734051018973e-06\\
41	9.09040333607037e-06\\
42	8.98934364943858e-06\\
};
\addplot [color=blue, dashed, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0\\
5	1.56358589890643e-09\\
6	2.04428152051469e-08\\
7	1.09234727747626e-07\\
8	3.68164214947203e-07\\
9	9.2672504592784e-07\\
10	1.90487207544056e-06\\
11	3.37592506491108e-06\\
12	5.34241257789604e-06\\
13	7.72929128861811e-06\\
14	1.03949310595002e-05\\
15	1.31548157499339e-05\\
16	1.58104018776612e-05\\
17	1.81763580771193e-05\\
18	2.010173363163e-05\\
19	2.14831308457692e-05\\
20	2.22698952641729e-05\\
21	2.2462492699664e-05\\
22	2.21058553826286e-05\\
23	2.12796784164911e-05\\
24	2.00874109783955e-05\\
25	1.86452185405217e-05\\
26	1.707174939435e-05\\
27	1.54792073121989e-05\\
28	1.39659997390602e-05\\
29	1.26110862255093e-05\\
30	1.14701112000113e-05\\
31	1.05734588480728e-05\\
32	9.92642864021833e-06\\
33	9.5116632593571e-06\\
34	9.29371794193876e-06\\
35	9.22535968415138e-06\\
36	9.25486828780541e-06\\
37	9.33336377798576e-06\\
38	9.42124422833681e-06\\
39	9.49294592653739e-06\\
40	9.53911276545977e-06\\
41	9.56376863863276e-06\\
42	9.57785557131989e-06\\
};
\addplot [color=black, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
1	0\\
2	0\\
3	0\\
4	0\\
5	1.56358589890643e-09\\
6	2.04428152051469e-08\\
7	1.09234727747626e-07\\
8	3.68168205961438e-07\\
9	9.27281234762562e-07\\
10	1.91145135516548e-06\\
11	3.40879056772933e-06\\
12	5.44572300598659e-06\\
13	7.971517264504e-06\\
14	1.08585040489373e-05\\
15	1.39185138947682e-05\\
16	1.69300852596759e-05\\
17	1.96691223012474e-05\\
18	2.19367434617754e-05\\
19	2.35803454289946e-05\\
20	2.45061905521173e-05\\
21	2.46835600377287e-05\\
22	2.41416559739151e-05\\
23	2.29610081359834e-05\\
24	2.12612696854193e-05\\
25	1.91871658830581e-05\\
26	1.68941221397472e-05\\
27	1.45348163394074e-05\\
28	1.22476180977682e-05\\
29	1.01476002925824e-05\\
30	8.3205270594167e-06\\
31	6.81994313078142e-06\\
32	5.66723633799641e-06\\
33	4.85432827713827e-06\\
34	4.3485000949636e-06\\
35	4.09884369534424e-06\\
36	4.04377316168245e-06\\
37	4.11902716122121e-06\\
38	4.2658257824129e-06\\
39	4.43830588859619e-06\\
40	4.6086675958643e-06\\
41	4.76725122206518e-06\\
42	4.91678351217044e-06\\
};
\end{axis}

\begin{axis}[%
width=7.812in,
height=3.125in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
